Completed Feature Disentanglement Learning for Multimodal MRIs Analysis

Multimodal MRIs play a crucial role in clinical diagnosis and treatment. Feature disentanglement (FD)-based methods, aiming at learning superior feature representations for multimodal data analysis, have achieved significant success in multimodal learning (MML). Typically, existing FD-based methods separate multimodal data into modality-shared and modality-specific features, and employ concatenation or attention mechanisms to integrate these features. However, our preliminary experiments indicate that these methods could lead to a loss of shared information among subsets of modalities when the inputs contain more than two modalities, and such information is critical for prediction accuracy. Furthermore, these methods do not adequately interpret the relationships between the decoupled features at the fusion stage. To address these limitations, we propose a novel Complete Feature Disentanglement (CFD) strategy that recovers the lost information during feature decoupling. Specifically, the CFD strategy not only identifies modality-shared and modality-specific features, but also decouples shared features among subsets of multimodal inputs, termed as modality-partial-shared features. We further introduce a new Dynamic Mixture-of-Experts Fusion (DMF) module that dynamically integrates these decoupled features, by explicitly learning the local-global relationships among the features. The effectiveness of our approach is validated through classification tasks on three multimodal MRI datasets. Extensive experimental results demonstrate that our approach outperforms other state-of-the-art MML methods with obvious margins, showcasing its superior performance.

==> figures_tex/completed_information_threemodals.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/completed_information_threemodals.pdf}
    \caption{
    Illustrations of incomplete feature representations in existing FD methods in the three-modal case. Sub-figure (a) shows a concept map, while sub-figure (b) presents an example from the MEN dataset. In (b), tumor and edema areas are marked with red and green boxes, respectively, and the yellow box highlights regions of high cell density in the tumor. Tumor and edema location information is shared across all three MRI series. Tumor characteristics are shared between T1C and FLAIR-C, edema characteristics between FLAIR-C and ADC, and cell density information between T1C and ADC.}
    
    % Illustrations of incompleted feature representation for existing feature disentanglement methods in the three-modal case. Sub-figure (a) presents a concept map, (b) shows a case in the MEN dataset. In sub-figure (b), the tumor and edema areas are enclosed within the red and the green boxes respectively, and the yellow box indicates high cell density in tumor area. Notably, the location information of tumor and edema is shared across all three MRI series. Additionally, the tumor characteristic information is shared between the T1C and FLAIR-C series, the edema characteristics are shared between the FLAIR-C and ADC series, while the information regarding the cell density in tumor area is shared between the T1C and ADC series.
    
    % \caption{Illustration of incompleted feature representation of existing feature disentanglement methods with three-modal as inputs. (a) is a concept map and (b) shows a case in the Meningiomas dataset. In (b), the tumor area is framed in the red box, the edema area is framed in the green box, and the yellow box contains a high cell density area. The location information of tumor and edema is shared among all three MRI series. The information about the tumor characteristic is shared by T1C and FLAIR-C series. Both FLAIR-C and ADC series share information about the edema characteristics. The information about the cell density of tumor area is shared between T1C and ADC series.}
    
    % \caption{Explanation of incomplete feature representation on previous feature disentanglement (FD) methods with three modalities. The upper part is a concept map. Different circles represent the feature spaces of different modals. Previous FD methods could decouple shared feature between all modals (yellow area) and specific features (green area). But they lost shared features between two modals (blue area) during feature decoupling. The lower part is an example in MEN dataset. The tumor area framed in red box is shared between T1C and Flair-C and the edema area framed in green box is shared between Flair-C and ADC. The information of two important area which play important roles in prediction are all lost in previous FD methods. \textcolor{red}{For the above figure, add more content in the circle, such as dot, to represent information/features}}
    \label{completed_information_threemodals}
\end{figure}

% subfigure
% \begin{figure}[ht]
% \centering
%     \subfigure[Concept map]{%
%         \includegraphics[width=0.75\linewidth]{figures/completed_information_threemodals_conceptmap.pdf}}
%     \quad
%     \subfigure[A case in Meningiomas Grade and Invasion Prediction dataset]{%
%         \includegraphics[width=0.8\linewidth]{figures/completed_information_threemodals_onecase.pdf}}
% %
% \caption{Explanation of incomplete feature representation on existing FD methods with three modals input. (a) is a concept map and (b) shows a case in Meningiomas Grade and Invasion Prediction dataset. In (b), the tumor area is framed in red box, the edema area is framed in green box, and the yellow box contains high cell density area.}
% \label{completed_information_threemodals}
% \end{figure}

==> figures_tex/param.tex <==
\begin{figure*}[ht]
\centering
    \subfigure[Parameter comparison]{%
        \includegraphics[width=0.47\linewidth]{figures/Param.pdf}}
    \quad
    \subfigure[GFLOPS comparison]{%
        \includegraphics[width=0.47\linewidth]{figures/GFLOPS.pdf}}
%
% \caption{Visualization results of contrast framework and proposed framework on MRNet and MEN datasets. The difference between the contrast and the proposed framework is whether the losses related to FD ($L_{sh}$, $L_{sup}$ and $L_{diff}$) work (the parameters $\alpha$ and $\beta$ equal to 0 means loss do not work). The right part contains t-SNE visualization of the decoupled features and heatmap which displys the cosine similarity of between any two decoupled features of proposed framework. And the left part contains t-SNE visualization and heatmap of contrast framework. In the heatmaps, the higher the value, the greater the similarity between two features.}
\caption{The computational complexity comparison including parameter and GFLOPS between proposed and comparison methods in the three-modal case and four-modal case.
}
\label{Param}
\end{figure*}

==> tables_tex/param.tex <==
\begin{table}[t]
	\centering
	\caption{The computational complexity comparison between proposed and comparison methods in the three-modal case and four-modal case.}
	\label{param}
	\Large
	\resizebox{0.45\textwidth}{!}{
		\begin{tabular}{ccccc}
			\hline
			\multirow{2}{*}{Methods} & \multicolumn{2}{c}{Three-modal} & \multicolumn{2}{c}{Four-modal} \\ \cline{2-5} 
			& Parameters (M)        & GFLOPS       & Parameters (M)       & GFLOPS       \\ \hline
			EmbraceNet~\cite{choi2019embracenet}               & 99.62            & 46.16        & 132.78          & 32.23        \\
			MISA~\cite{hazarika2020misa}                     & 100.72           & 46.17        & 134.22          & 45.44        \\
			MAML~\cite{zhang2021modality}                     & 202.61           & 165.63       & 270.09          & 111.93       \\
			ETMC~\cite{han2022trusted}                     & 101.62           & 46.17        & 135.44          & 45.44        \\
			ADCCA~\cite{zhou2023attentive}                    & 99.93            & 46.16        & 133.24          & 45.44        \\
			DMD~\cite{li2023decoupled}                      & 104.22           & 46.27        & 142.75          & 45.67        \\ 
                CCML~\cite{liu2024dynamic}                      & 99.90           & 46.16        & 133.20          & 32.23        \\
                GLoMo~\cite{zhuang2024glomo}                      & 101.68           & 46.29        & 135.31          & 32.32        \\\hline
			Proposed                 & 99.62            & 46.16        & 132.89          & 45.44        \\ \hline
		\end{tabular}}
\end{table}
